Anytime-valid sequential testing for elicitable functionals via supermartingales

We design sequential tests for a large class of nonparametric null hypotheses based on elicitable and identifiable functionals. Such functionals are defined in terms of scoring functions and identification functions, which are ideal building blocks for constructing nonnegative supermartingales under the null. This in turn yields sequential tests via Ville's inequality. Using regret bounds from Online Convex Optimization, we obtain rigorous guarantees on the asymptotic power of the tests for a wide range of alternative hypotheses. Our results allow for bounded and unbounded data distributions, assuming that a sub-$\psi$ tail bound is satisfied.

==> submission_2022-04-12/arxiv/symdefs.tex <==
% % THEOREMS STYLE --------------------------------------------------
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{conjecture}[theorem]{Conjecture}

% \theoremstyle{definition}
% \newtheorem{exercise}[theorem]{Exercise}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{problem}[theorem]{Problem}
% %\theoremstyle{remark}
% \newtheorem{remark}[theorem]{\textbf{Remark}}
% \newtheorem{example}[theorem]{\textbf{Example}}
%\numberwithin{equation}{section}
%\numberwithin{theorem}{section}



\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother



% MATH NEW COMMAND --------------------------------------------------
\renewcommand{\d}{{\rm d}}
\newcommand{\e}{{\rm e}}
\renewcommand{\k}{{\bf k}}
\newcommand{\I}{{\mathbb I}}
\renewcommand{\P}{{\mathbb P}}
% \newcommand{\C}{{\mathbb C}}
\newcommand{\E}{{\mathbb E}}
% \newcommand{\F}{{\mathbb F}}
% \newcommand{\G}{{\mathbb G}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
% \renewcommand{\S}{{\mathbb S}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\V}{{\mathbb V}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Acal}{{\mathcal A}}
\newcommand{\Bcal}{{\mathcal B}}
\newcommand{\Ccal}{{\mathcal C}}
\newcommand{\Dcal}{{\mathcal D}}
\newcommand{\Ecal}{{\mathcal E}}
\newcommand{\Fcal}{{\mathcal F}}
\newcommand{\Gcal}{{\mathcal G}}
\newcommand{\Hcal}{{\mathcal H}}
\newcommand{\Ical}{{\mathcal I}}
\newcommand{\Jcal}{{\mathcal J}}
\newcommand{\Kcal}{{\mathcal K}}
\newcommand{\Lcal}{{\mathcal L}}
\newcommand{\Ucal}{{\mathcal U}}
\newcommand{\Mcal}{{\mathcal M}}
\newcommand{\Ncal}{{\mathcal N}}
\newcommand{\Ocal}{{\mathcal O}}
\newcommand{\Pcal}{{\mathcal P}}
\newcommand{\Qcal}{{\mathcal Q}}
\newcommand{\Rcal}{{\mathcal R}}
\newcommand{\Scal}{{\mathcal S}}
\newcommand{\Tcal}{{\mathcal T}}
\newcommand{\Vcal}{{\mathcal V}}
\newcommand{\Wcal}{{\mathcal W}}
\newcommand{\Xcal}{{\mathcal X}}
\newcommand{\Ycal}{{\mathcal Y}}
\newcommand{\Zcal}{{\mathcal Z}}

\newcommand{\Var}{{\rm Var}}

\newcommand{\midd}{{\ \bigg|\ }}
\newcommand{\Mid}{{\ \Big|\ }}
\newcommand{\Midd}{{\ \Bigg|\ }}

\newcommand{\fdot}{{\,\cdot\,}}
\newcommand{\id}{{\rm id}}
\newcommand{\ind}{\mathds{1}}

\DeclareMathOperator{\sgn}{\mathsf{sgn}}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\maximize}{maximize}

\DeclareMathOperator{\dotp}{{\bm\cdot}}
\DeclareMathOperator{\VaR}{{VaR}}
\DeclareMathOperator{\RVaR}{{RVaR}}


\DeclareMathOperator{\Max}{Max}


% DOCUMENT SPECIFIC COMMANDS ----------------------------------------

\usepackage{tikz}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

\newcommand{\pist}{\pi^{\ast}}
\newcommand{\Pfr}{\mathfrak{P}}
\newcommand{\Pfrh}{\widehat{\Pfr}}

\newcommand{\lambdap}{{\lambda^{\prime}}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bs}{\mathbf{s}}

\newcommand{\Qrl}{Q_{\text{real}}}
\newcommand{\bl}{\bf \lambda}

\newcommand{\mh}{\hat{m}}
\newcommand{\Ch}{\hat{C}}

\newcommand{\Eh}{\hat\E}
\newcommand{\reg}{\text{Regret}}

\DeclareMathOperator{\diam}{diam}

\newcommand{\Hnull}{\Hcal_0}
\newcommand{\rbox}[1]{{\color{red} \fbox{#1}}}


\newcommand{\umax}{u_{\max}}
\newcommand{\Abd}{A^{\mathrm{bd}}}
\newcommand{\Apsi}{A^{\psi}}

==> submission_2022-04-12/bernoulli/symdefs.tex <==
% % THEOREMS STYLE --------------------------------------------------
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{conjecture}[theorem]{Conjecture}

% \theoremstyle{definition}
% \newtheorem{exercise}[theorem]{Exercise}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{problem}[theorem]{Problem}
% %\theoremstyle{remark}
% \newtheorem{remark}[theorem]{\textbf{Remark}}
% \newtheorem{example}[theorem]{\textbf{Example}}
%\numberwithin{equation}{section}
%\numberwithin{theorem}{section}



\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother



% MATH NEW COMMAND --------------------------------------------------
\renewcommand{\d}{{\rm d}}
\newcommand{\e}{{\rm e}}
\renewcommand{\k}{{\bf k}}
\newcommand{\I}{{\mathbb I}}
\renewcommand{\P}{{\mathbb P}}
% \newcommand{\C}{{\mathbb C}}
\newcommand{\E}{{\mathbb E}}
% \newcommand{\F}{{\mathbb F}}
% \newcommand{\G}{{\mathbb G}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
% \renewcommand{\S}{{\mathbb S}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\V}{{\mathbb V}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Acal}{{\mathcal A}}
\newcommand{\Bcal}{{\mathcal B}}
\newcommand{\Ccal}{{\mathcal C}}
\newcommand{\Dcal}{{\mathcal D}}
\newcommand{\Ecal}{{\mathcal E}}
\newcommand{\Fcal}{{\mathcal F}}
\newcommand{\Gcal}{{\mathcal G}}
\newcommand{\Hcal}{{\mathcal H}}
\newcommand{\Ical}{{\mathcal I}}
\newcommand{\Jcal}{{\mathcal J}}
\newcommand{\Kcal}{{\mathcal K}}
\newcommand{\Lcal}{{\mathcal L}}
\newcommand{\Ucal}{{\mathcal U}}
\newcommand{\Mcal}{{\mathcal M}}
\newcommand{\Ncal}{{\mathcal N}}
\newcommand{\Ocal}{{\mathcal O}}
\newcommand{\Pcal}{{\mathcal P}}
\newcommand{\Qcal}{{\mathcal Q}}
\newcommand{\Rcal}{{\mathcal R}}
\newcommand{\Scal}{{\mathcal S}}
\newcommand{\Tcal}{{\mathcal T}}
\newcommand{\Vcal}{{\mathcal V}}
\newcommand{\Wcal}{{\mathcal W}}
\newcommand{\Xcal}{{\mathcal X}}
\newcommand{\Ycal}{{\mathcal Y}}
\newcommand{\Zcal}{{\mathcal Z}}

\newcommand{\Var}{{\rm Var}}

\newcommand{\midd}{{\ \bigg|\ }}
\newcommand{\Mid}{{\ \Big|\ }}
\newcommand{\Midd}{{\ \Bigg|\ }}

\newcommand{\fdot}{{\,\cdot\,}}
\newcommand{\id}{{\rm id}}
\newcommand{\ind}{\mathds{1}}

\DeclareMathOperator{\sgn}{\mathsf{sgn}}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\maximize}{maximize}

\DeclareMathOperator{\dotp}{{\bm\cdot}}
\DeclareMathOperator{\VaR}{{VaR}}
\DeclareMathOperator{\RVaR}{{RVaR}}


\DeclareMathOperator{\Max}{Max}


% DOCUMENT SPECIFIC COMMANDS ----------------------------------------

\usepackage{tikz}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

\newcommand{\pist}{\pi^{\ast}}
\newcommand{\Pfr}{\mathfrak{P}}
\newcommand{\Pfrh}{\widehat{\Pfr}}

\newcommand{\lambdap}{{\lambda^{\prime}}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bs}{\mathbf{s}}

\newcommand{\Qrl}{Q_{\text{real}}}
\newcommand{\bl}{\bf \lambda}

\newcommand{\mh}{\hat{m}}
\newcommand{\Ch}{\hat{C}}

\newcommand{\Eh}{\hat\E}
\newcommand{\reg}{\text{Regret}}

\DeclareMathOperator{\diam}{diam}

\newcommand{\Hnull}{\Hcal_0}
\newcommand{\rbox}[1]{{\color{red} \fbox{#1}}}


\newcommand{\umax}{u_{\max}}
\newcommand{\Abd}{A^{\mathrm{bd}}}
\newcommand{\Apsi}{A^{\psi}}
